Cooperative UWB-Based Localization for Outdoors Positioning and Navigation of UAVs aided by Ground Robots

Unmanned aerial vehicles (UAVs) are becoming largely ubiquitous with an increasing demand for aerial data. Accurate navigation and localization, required for precise data collection in many industrial applications, often relies on RTK GNSS. These systems, able of centimeter-level accuracy, require a setup and calibration process and are relatively expensive. This paper addresses the problem of accurate positioning and navigation of UAVs through cooperative localization. Inexpensive ultra-wideband (UWB) transceivers installed on both the UAV and a support ground robot enable centimeter-level relative positioning. With fast deployment and wide setup flexibility, the proposed system is able to accommodate different environments and can also be utilized in GNSS-denied environments. Through extensive simulations and test fields, we evaluate the accuracy of the system and compare it to GNSS in urban environments where multipath transmission degrades accuracy. For completeness, we include visual-inertial odometry in the experiments and compare the performance with the UWB-based cooperative localization.

==> fig/uwb_gps_vio_error_boxplot.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.91796875,0.25,0.203125}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.6328125,0.203125,0.91796875}
\definecolor{color3}{rgb}{0.171875,0.49609375,0.71875}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
            height=\figureheight,
            width=\figurewidth,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=2.5, xmax=5.5,
xtick={3,4,5}, 
xticklabels={VIO-X,VIO-Y,VIO-Z},
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={y/m},
ymajorgrids,
ymin=-0.2041598322165, ymax=4.2888497382065,
ytick style={color=black}
]
\addplot [line width=2pt, color0]
table {%
2.85 0.14334829911975
3.15 0.14334829911975
3.15 0.313649677813772
3.075 0.340273547968
3.15 0.366897418122227
3.15 0.703215187335025
2.85 0.703215187335025
2.85 0.366897418122227
2.925 0.340273547968
2.85 0.313649677813772
2.85 0.14334829911975
};
\addplot [black]
table {%
3 0.14334829911975
3 0.000565849789999906
};
\addplot [black]
table {%
3 0.703215187335025
3 1.5407297163
};
\addplot [black]
table {%
2.925 0.000565849789999906
3.075 0.000565849789999906
};
\addplot [black]
table {%
2.925 1.5407297163
3.075 1.5407297163
};
\addplot [line width=2pt, color2]
table {%
3.85 0.23068461689975
4.15 0.23068461689975
4.15 0.421681808783881
4.075 0.443865155955
4.15 0.466048503126119
4.15 0.6971728276275
3.85 0.6971728276275
3.85 0.466048503126119
3.925 0.443865155955
3.85 0.421681808783881
3.85 0.23068461689975
};
\addplot [black]
table {%
4 0.23068461689975
4 6.78755300000944e-05
};
\addplot [black]
table {%
4 0.6971728276275
4 1.37052999886
};
\addplot [black]
table {%
3.925 6.78755300000944e-05
4.075 6.78755300000944e-05
};
\addplot [black]
table {%
3.925 1.37052999886
4.075 1.37052999886
};
\addplot [line width=2pt, color3]
table {%
4.85 0.2863183199475
5.15 0.2863183199475
5.15 0.366798369904502
5.075 0.47536206777
5.15 0.583925765635498
5.15 2.5692779101575
4.85 2.5692779101575
4.85 0.583925765635498
4.925 0.47536206777
4.85 0.366798369904502
4.85 0.2863183199475
};
\addplot [black]
table {%
5 0.2863183199475
5 0.0066105721099996
};
\addplot [black]
table {%
5 2.5692779101575
5 4.08462203046
};
\addplot [black]
table {%
4.925 0.0066105721099996
5.075 0.0066105721099996
};
\addplot [black]
table {%
4.925 4.08462203046
5.075 4.08462203046
};
\addplot [color1]
table {%
2.925 0.340273547968
3.075 0.340273547968
};
\addplot [color1]
table {%
3.925 0.443865155955
4.075 0.443865155955
};
\addplot [color1]
table {%
4.925 0.47536206777
5.075 0.47536206777
};

\nextgroupplot[
            height=\figureheight,
            width=\figurewidth,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=2.5, xmax=5.5,
xtick={3,4,5}, 
xticklabels={UWB-X,UWB-Y,UWB-Z},
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={y/m},
ymajorgrids,
ymin=-0.16549055, ymax=3.48031755,
ytick style={color=black}
]
\addplot [line width=2pt, color0]
table {%
2.85 0.3525635
3.15 0.3525635
3.15 0.663919851384457
3.075 0.7092355
3.15 0.754551148615543
3.15 1.30549525
2.85 1.30549525
2.85 0.754551148615543
2.925 0.7092355
2.85 0.663919851384457
2.85 0.3525635
};
\addplot [black]
table {%
3 0.3525635
3 0.000228000000000117
};
\addplot [black]
table {%
3 1.30549525
3 2.730964
};
\addplot [black]
table {%
2.925 0.000228000000000117
3.075 0.000228000000000117
};
\addplot [black]
table {%
2.925 2.730964
3.075 2.730964
};
\addplot [line width=2pt, color2]
table {%
3.85 0.32147575
4.15 0.32147575
4.15 0.579247862826431
4.075 0.6363865
4.15 0.693525137173569
4.15 1.52303025
3.85 1.52303025
3.85 0.693525137173569
3.925 0.6363865
3.85 0.579247862826431
3.85 0.32147575
};
\addplot [black]
table {%
4 0.32147575
4 0.00053700000000001
};
\addplot [black]
table {%
4 1.52303025
4 3.314599
};
\addplot [black]
table {%
3.925 0.00053700000000001
4.075 0.00053700000000001
};
\addplot [black]
table {%
3.925 3.314599
4.075 3.314599
};
\addplot [line width=2pt, color3]
table {%
4.85 0.12925575
5.15 0.12925575
5.15 0.271720993925497
5.075 0.291425
5.15 0.311129006074503
5.15 0.543606500000001
4.85 0.543606500000001
4.85 0.311129006074503
4.925 0.291425
4.85 0.271720993925497
4.85 0.12925575
};
\addplot [black]
table {%
5 0.12925575
5 0.000409999999999577
};
\addplot [black]
table {%
5 0.543606500000001
5 1.136963
};
\addplot [black]
table {%
4.925 0.000409999999999577
5.075 0.000409999999999577
};
\addplot [black]
table {%
4.925 1.136963
5.075 1.136963
};
\addplot [color1]
table {%
2.925 0.7092355
3.075 0.7092355
};
\addplot [color1]
table {%
3.925 0.6363865
4.075 0.6363865
};
\addplot [color1]
table {%
4.925 0.291425
5.075 0.291425
};

\nextgroupplot[
            height=\figureheight,
            width=\figurewidth,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=2.5, xmax=5.5,
xtick={3,4,5}, 
xticklabels={GPS-X,GPS-Y,GPS-Z},
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={y/m},
ymajorgrids,
ymin=-1.98942987402609, ymax=41.8011407864614,
ytick style={color=black}
]
\addplot [line width=2pt, color0]
table {%
2.85 2.29513189908015
3.15 2.29513189908015
3.15 3.50118807088244
3.075 3.73463416107142
3.15 3.96808025126039
3.15 7.20421293512076
2.85 7.20421293512076
2.85 3.96808025126039
2.925 3.73463416107142
2.85 3.50118807088244
2.85 2.29513189908015
};
\addplot [black]
table {%
3 2.29513189908015
3 0.00105061054152111
};
\addplot [black]
table {%
3 7.20421293512076
3 14.4110150642539
};
\addplot [black]
table {%
2.925 0.00105061054152111
3.075 0.00105061054152111
};
\addplot [black]
table {%
2.925 14.4110150642539
3.075 14.4110150642539
};
\addplot [line width=2pt, color2]
table {%
3.85 1.89610601252667
4.15 1.89610601252667
4.15 3.17713051610494
4.075 3.30582850812832
4.15 3.4345265001517
4.15 4.60246477615834
3.85 4.60246477615834
3.85 3.4345265001517
3.925 3.30582850812832
3.85 3.17713051610494
3.85 1.89610601252667
};
\addplot [black]
table {%
4 1.89610601252667
4 0.00318968972726463
};
\addplot [black]
table {%
4 4.60246477615834
4 8.54358799637033
};
\addplot [black]
table {%
3.925 0.00318968972726463
4.075 0.00318968972726463
};
\addplot [black]
table {%
3.925 8.54358799637033
4.075 8.54358799637033
};
\addplot [line width=2pt, color3]
table {%
4.85 4.62876387283643
5.15 4.62876387283643
5.15 9.05131237161907
5.075 9.72946982217759
5.15 10.4076272727361
5.15 18.8895719133201
4.85 18.8895719133201
4.85 10.4076272727361
4.925 9.72946982217759
4.85 9.05131237161907
4.85 4.62876387283643
};
\addplot [black]
table {%
5 4.62876387283643
5 0.0193616773566083
};
\addplot [black]
table {%
5 18.8895719133201
5 39.8106603018938
};
\addplot [black]
table {%
4.925 0.0193616773566083
5.075 0.0193616773566083
};
\addplot [black]
table {%
4.925 39.8106603018938
5.075 39.8106603018938
};
\addplot [color1]
table {%
2.925 3.73463416107142
3.075 3.73463416107142
};
\addplot [color1]
table {%
3.925 3.30582850812832
4.075 3.30582850812832
};
\addplot [color1]
table {%
4.925 9.72946982217759
5.075 9.72946982217759
};
\end{groupplot}

\end{tikzpicture}

